hp-finite-elements for simulating electromagnetic fields in optical devices with rough textures

The finite-element method is a preferred numerical method when electromagnetic fields at high accuracy are to be computed in nano-optics design. Here, we demonstrate a finite-element method using hp-adaptivity on tetrahedral meshes for computation of electromagnetic fields in a device with rough textures. The method allows for efficient computations on meshes with strong variations in element sizes. This enables to use precise geometry resolution of the rough textures. Convergence to highly accurate results is observed.

==> osd15_burger_bibliography.tex <==
\nopagebreak
\begin{thebibliography}{10}

\bibitem{Taflove2005computational}
Taflove, A. and Hagness, S.~C.,  [{\em Computational
  electrodynamics}{\nolinebreak\hspace{0.1em}]}, Artech house (2005).

\bibitem{Jin2014finite}
Jin, J.-M.,  [{\em The finite element method in
  electromagnetics}{\nolinebreak\hspace{0.1em}]}, John Wiley \& Sons (2014).

\bibitem{Lavrinenko2014crc}
Lavrinenko, A.~V., et al.,  [{\em Numerical Methods in
  Photonics}{\nolinebreak\hspace{0.1em}]}, CRC Press (2014).

\bibitem{Maes2013oe}
Maes, B., et al., ``Simulations of high-{Q} optical nanocavities with a gradual
  {1D} bandgap,'' {\em Opt. Express}~{\bf 21},  6794 (2013).

\bibitem{Hoffmann2009spie}
Hoffmann, J., et al., ``Comparison of electromagnetic field solvers for the {3D} analysis of
  plasmonic nano antennas,'' {\em Proc. SPIE}~{\bf 7390},  73900J (2009).

\bibitem{Bock2013lpr}
Bock, M., et al., 
 ``Nanostructured fibers
  for sub-10 fs optical pulse delivery,'' {\em Laser Photon. Rev.}~{\bf 7},
  566 (2013).

\bibitem{wong2012excitation}
Wong, G. K.~L., et al., 
 ``Excitation of orbital angular momentum resonances in
  helically twisted photonic crystal fiber,'' {\em Science}~{\bf 337},  446
  (2012).

\bibitem{paetzold2011design}
Paetzold, U.~W., et al., 
``Design
  of nanostructured plasmonic back contacts for thin-film silicon solar
  cells,'' {\em Optics Express}~{\bf 19},  A1219 (2011).

\bibitem{Tyminski2013al}
Tyminski, J.~K., et al., 
  ``Topographic mask modeling with reduced basis finite element method,'' {\em
  Proc. SPIE}~{\bf 8683},  86831C (2013).

\bibitem{Gschrey2015nc}
Gschrey, M., et al., 
``Highly indistinguishable
  photons from deterministic quantum-dot microlenses utilizing
  three-dimensional in situ electron-beam lithography,'' {\em Nat.
  Commun.}~{\bf 6},  7662 (2015).

\bibitem{Kaschke2014oe}
Kaschke, J., et al., 
 ``Tapered n-helical
  metamaterials with three-fold rotational symmetry as improved circular
  polarizers,'' {\em Opt. Express}~{\bf 22},  19936 (2014).

\bibitem{Shchukin2014ieee}
Shchukin, V., et al., 
 ``Single-mode vertical cavity surface emitting laser via
  oxide-aperture-engineering of leakage of high-order transverse modes,'' {\em
  IEEE J. Quantum Electron.}~{\bf 50},  990 (2014).

\bibitem{Karl2009OE}
Karl, M., et al., 
  ``Dependencies of micro-pillar cavity quality factors calculated with finite
  element methods,'' {\em Optics Express}~{\bf 17},  1144 (2009).

\bibitem{Kewes2013design}
Kewes, G., et al., 
 ``Design and numerical optimization of an easy-to-fabricate
  photon-to-plasmon coupler for quantum plasmonics,'' {\em Appl. Phys.
  Lett.}~{\bf 102},  051104 (2013).

\bibitem{Bodermann2012op}
Bodermann, B., et al., 
 ``First steps towards a
  scatterometry reference standard,'' {\em Proc. SPIE}~{\bf 8466},  84660E
  (2012).

\bibitem{Burger2013pw}
Burger, S., et al., 
  ``Advanced finite-element methods for design and analysis of nano-optical
  structures: Applications,'' {\em Proc. SPIE}~{\bf 8642},  864205 (2013).

\bibitem{MON03}
Monk, P.,  [{\em Finite Element Methods for Maxwell's
  Equations}{\nolinebreak\hspace{0.1em}]}, Oxford University Press (2003).

\bibitem{Babuska1981}
Babu\v{s}ka, I. and Dorr, M.~R., ``Error estimates for the combined h and p
  versions of the finite element method,'' {\em Numer. Math.}~{\bf 37}(2),
  257--277 (1981).

\bibitem{Pomplun2007pssb}
Pomplun, J., et al., 
``Adaptive finite
  element method for simulation of optical nano structures,'' {\em phys. stat.
  sol. (b)}~{\bf 244},  3419 (2007).

\bibitem{Burger2015al}
Burger, S., et al., 
  ``Hp-finite element method for simulating light scattering from complex {3D}
  structures,'' {\em Proc. SPIE}~{\bf 9424},  94240Z (2015).

\bibitem{Battaglia2012acsn}
Battaglia, C., et al., 
 ``Light trapping in solar cells: Can periodic beat
  random?,'' {\em ACS Nano}~{\bf 6}(3),  2790 (2012).

\bibitem{Schaedle_jcp_2007}
Sch\"adle, et al.,
  ``Domain decomposition method for {M}axwell's equations: {S}cattering off
  periodic structures,'' {\em J. Comp. Phys.}~{\bf 226},  447 (2007).

\bibitem{Ding2011semsc}
Ding, K., et al., 
``Characterization and simulation
  of a-{S}i:{H}/uc-{S}i:{H} tandem solar cells,'' {\em Sol. Energ. Mat. Sol.
  Cells}~{\bf 95},  3318 (2011).

\bibitem{Palik1985}
Palik, E.~D.,  [{\em Handbook of optical constants of
  solids}{\nolinebreak\hspace{0.1em}]}, Academic press (1985).

\bibitem{Lockau2011rigorous}
Lockau, D., et al., 
  ``Rigorous optical simulation of light management in crystalline silicon thin
  film solar cells with rough interface textures,'' {\em Proc. SPIE}~{\bf
  7933},  79330M (2011).

\bibitem{Wiesendanger2014apl}
Wiesendanger, S., et al., 
``Effects of film growth modes on light trapping in
  silicon thin film solar cells,'' {\em Appl. Phys. Lett.}~{\bf 104}(23),
  231103 (2014).

\end{thebibliography}

